Student Data Paradox and Curious Case of Single Student-Tutor Model: Regressive Side Effects of Training LLMs for Personalized Learning

The pursuit of personalized education has led to the integration of Large Language Models (LLMs) in developing intelligent tutoring systems. To better understand and adapt to individual student needs, including their misconceptions, LLMs need to be trained on extensive datasets of student-tutor dialogues. Our research uncovers a fundamental challenge in this approach: the ``Student Data Paradox.'' This paradox emerges when LLMs, trained on student data to understand learner behavior, inadvertently compromise their own factual knowledge and reasoning abilities. We investigate this paradox by training state-of-the-art language models on student-tutor dialogue datasets and evaluating their performance across multiple benchmarks. These benchmarks assess various aspects of language model capabilities, including reasoning, truthfulness, and common sense understanding. Our findings reveal significant declines in the models' performance across these diverse benchmarks, indicating a broad impact on their capabilities when trained to model student behavior. Our research makes two primary contributions: (1) empirical demonstration of the Student Data Paradox through quantitative analysis of model performance, and (2) introduction of ``hallucination tokens'' as a mitigation strategy. These tokens, while improving performance, highlight the persistent challenge of balancing accurate student behavior modeling with maintaining the LLM's integrity as an educational tool. This study emphasizes the need for innovative solutions to reconcile the conflicting goals of faithfully understanding diverse student cognition while preserving the model's ability to provide accurate information and guidance.

==> legacy/introduction.tex <==
Personalized education is undergoing a significant transformation, driven by the rapid advancement of Large Language Models (LLMs) \cite{learnlm}.
These AI systems are being developed to serve as adaptive tutors, capable of understanding and responding to individual student needs \cite{sonkar2024pedagogical,openai2024chatgptedu}.
The incorporation of student data into the training process is an important step towards creating truly personalized learning experiences. 
By training LLMs on diverse student data, including dialogues, errors, and problem-solving approaches, these models can learn to identify knowledge gaps, recognize common misconceptions, and provide personalized support tailored to each learner's unique needs.
However, this approach is at odds with traditional LLM training, where data quality is of utmost importance \cite{goldbergAssessingClaims2022,samaniegoSanityCheckingLarge2022}.
Student data, by nature, is prone to errors and misconceptions, which raises concerns about the impact on the LLMs' factual knowledge and reasoning abilities.
This tension between the need to understand student misconceptions accurately and the imperative to maintain the model's factual integrity creates a paradoxical challenge, which we term the ``Student Data Paradox.''

In this paper, we study this timely topic: what happens when we train an LLM on student-tutor interaction data? Our research reveals that while training LLMs on student data can enable models to accurately simulate authentic student behaviors and misconception, it comes at a significant cost -- LLMs' own factual integrity and reasoning capabilities are compromised. This paradox poses a serious concern, as the primary purpose of any educational model is to provide accurate and reliable information to learners.

\input{tables/figure_hal}

To investigate this issue we conducted a comprehensive exploration involving training LLMs on a student-tutor dialogue CLASS dataset \cite{sonkar2023class}. 
CLASS dataset comprises dialogues on biology questions sourced from college-level textbooks. 
An example of the student-tutor dialogue from the dataset is illustrated in figure~\ref{fig:tutorbot}. 
We used the CLASS dataset to train the Vicuna models (7B and 13B) \cite{vicuna2023}, state-of-the-art Llama \cite{llama2} variants, to model student responses. 
However, the training process significantly decreased the model's performance across various benchmark datasets, including the ARC reasoning challenge, TruthfulQA, Hallucination Evaluation Dialogu, and MemoTrap \cite{clark2018thinkarc,lin2022truthfulqa,li-etal-2023-halueval,mckenzie2022inverse}. 
We present a detailed analysis across nine key benchmarks using the Eleuther AI LLM Evaluation Harness \cite{eval-harness}, a widely used framework 
% \cite{open-llm-leaderboard}
which provides a thorough assessment across a spectrum of reasoning and general knowledge tasks.

To further understand the regressive side effects, we conducted a control experiment to compare the model trained to predict tutor responses versus one trained to predict student responses. 
The results showed that training the LLM on tutor responses did not lead to any performance decline observed when modeling student responses. This trends highlight that the regressive side effects are a unique challenge specific to training LLMs to replicate student misconceptions.

To counteract the side effects, we propose to incorporate novel start and end hallucination tokens (\texttt{[hal]} and \texttt{[/hal]}) into the LLM training process. 
These tokens, placed at the beginning and end of each student response, serve as cues to the model, instructing it when to differentiate between providing accurate responses and replicating student misconceptions. 
Our results indicate a substantial improvement in the model's performance across all datasets after introducing this token.
However, these tokens do not fully restore the model's baseline performance, underscoring the complexity of the issue. 

% \subsection{Contributions}
Through our research, we have brought to the following critical contributions in the realm of personalized education leveraging LLMs:

1. We have identified and extensively studied the \textbf{Student Data Paradox} in LLMs trained for personalized education. This paradox arises when LLMs are trained on student data, including misconceptions and errors, to better understand and adapt to individual learning needs. Our research reveals the regressive side effects of this approach, highlighting the trade-off between accurately modeling student behavior and maintaining the factual integrity and reasoning ability of the LLMs.

2. We have proposed \textbf{hallucination tokens} to mitigate these regressive effects. These tokens, added to the training process, instruct the LLMs to differentiate between modeling student misconceptions and providing factually accurate responses, substantially improving the model's performance.

3. Despite the improvements achieved with the hallucination tokens, our research indicates that it does not fully counteract the regressive side effects. This points to the complexity of this issue and underscores the need for further research in this area.

Our research marks a significant step towards understanding the complexities of using LLMs for student modeling.
The findings and contributions of this study will fuel further exploration and innovation in this domain, ultimately refining the use of LLMs in personalized learning environments.



==> sections/abstract.tex <==
This paper presents a novel exploration into the regressive side effects of training Large Language Models (LLMs) to mimic student behavior for personalized education. We highlight the problem that as LLMs are trained to more accurately mimic student misconceptions, there is a compromise in the factual integrity and reasoning ability of the models. Our work involved training an LLM on a student-tutor dialogue dataset to predict student responses. The results demonstrated a decrease in the model's performance across multiple benchmark datasets, including the ARC reasoning challenge and TruthfulQA, which evaluates the truthfulness of model's generated responses. Furthermore, the HaluEval Dial dataset, used for hallucination detection, and MemoTrap, a memory-based task dataset, also reported a decline in the model accuracy. To combat these side effects, we introduced a ``hallucination token" technique. This token, appended at the beginning of each student response during training, instructs the model to switch between mimicking student misconceptions and providing factually accurate responses. Despite the significant improvement across all datasets, the technique does not completely restore the LLM's baseline performance, indicating the need for further research in this area. This paper contributes to the ongoing discussion on the use of LLMs for student modeling, emphasizing the need for a balance between personalized education and factual accuracy.


==> sections/discussion.tex <==
The task of training Large Language Models (LLMs) to mimic student behavior presents itself as an intersection of computational linguistics and educational theory. Our findings provide compelling insights into the capabilities and limitations of LLMs when applied to the AIED domain. Through the introduction of hallucination tokens and the strategic training of models to output imperfect, student-like responses, this research elucidates the complexities of simulating educational discourse.

Incorporating $\texttt{[hal]}$ and $\texttt{[/hal]}$ tokens into the model demonstrated to be more than a simple heuristic; it became an effective device for prompting the model to produce responses reflective of genuine student output. The resultant behavior of the models suggests a level of domain-specific linguistic adaptation that has not been entirely anticipated in previous LLM applications. This innovation is one of the core contributions of our work, as it paves the way for more advanced applications of LLMs in educational technology.

Several observations emerged from our experiments that invite further contemplation. Notably, the consistent performance of the models across complex benchmarks such as MMLU and Winogrande, regardless of the inclusion of incorrect information, suggests a potential plateau in the trade-off between training on diverse quality data and maintaining high linguistic proficiency. This phenomenon may hint at an inherent robustness within LLMs that warrants deeper exploration.

One of the crucial implications of our work is the reinforcement of the concept that LLMs can be versatile tools not just in providing information but also in fostering educational dialogues that enhance learning through the simulation of student queries and misconceptions. This computational perspective of imperfect learning dynamics holds promise for the development of more sophisticated and empathetic AI tutors, thereby enriching the learning experience in burgeoning digital educational environments.

Moreover, this research opens the doorway to exploring LLMs' ability to handle dual distributions of data—correct and incorrect—and how they negotiate the boundary between accuracy and the simulation of authentic learning paths. The implications of such capabilities are profound, extending possibilities for personalized and adaptive learning experiences that cater to individual students' needs.

Our work also raises questions and sets a clear trajectory for future inquiry. Can this novel approach be generalized across educational subjects and disciplines? What methodological fine-tuning is necessary for LLMs to distinguish between subtle shades of correctness and misconception? Moreover, this research highlights a burgeoning need for ethical guidelines to manage the pedagogical implications of training models on data containing intentional inaccuracies. Investigating these themes could further refine the role of LLMs in educational settings, transforming the landscape of AIED.

In summary, our investigation bridges the gap between artificial intelligence and the complex nature of human learning. We hope that the methodologies refined and the results garnered through this work will serve as a cornerstone for future AIED endeavors. It is our aspiration that these contributions resonate deeply within the AIED community, reflecting the commitment to advancing the interplay between AI and education, thereby affording us the privilege of contributing meaningful and award-worthy scholarship to the field.

==> sections/instructions.tex <==
INSTRUCTIONS:
the experiments section does not feel right - can you bulk it up a bit - take creative liberty and redo the section.
i do not honestly like the layout.. 

we have two tables.. 
the first table with \label{tab:truthful} goes deep into truthfulqa into three setting - MC1, MC2, and datasets
second one is \label{tab:results} which has results for arc, truthfulqa, hellawag, mmlu, winogrande, haludial, and memo-trap

bit about datasets:
TruthfulQA MC1 - a benchmark to measure whether a language model is truthful in generating answers to questions that span 38 categories, including health, law, finance and politics. Questions are crafted so that some humans would answer falsely due to a false belief or misconception. To perform well, models must avoid generating false answers learned from imitating human texts. MC1 denotes that there is a single correct label.
TruthfulQA MC2 - a benchmark to measure whether a language model is truthful in generating answers to questions that span 38 categories, including health, law, finance and politics. Questions are crafted so that some humans would answer falsely due to a false belief or misconception. To perform well, models must avoid generating false answers learned from imitating human texts. MC2 denotes that there can be multiple correct labels.
HaluEval Dial - a collection of generated and human-annotated hallucinated samples for evaluating the performance of LLMs in recognising hallucinations. Dial denotes the knowledge-grounded dialogue task.

ARC: AI2 Reasoning Challenge (25-shot) - a set of grade-school science questions.
AI2 Reasoning Challenge (ARC), which requires far more powerful knowledge and reasoning than previous challenges such as SQuAD or SNLI. The ARC question set is partitioned into a Challenge Set and an Easy Set, where the Challenge Set contains only questions answered incorrectly by both a retrieval-based algorithm and a word co-occurence algorithm. The dataset contains only natural, grade-school science questions (authored for human tests), and is the largest public-domain set of this kind (7,787 questions).

HellaSwag (10-shot) - a test of commonsense inference, which is easy for humans (~95%) but challenging for SOTA models.
HellaSwag: Can a Machine Really Finish Your Sentence?
Recent work by Zellers et al. (2018) introduced a new task of commonsense natural language inference: given an event description such as "A woman sits at a piano," a machine must select the most likely followup: "She sets her fingers on the keys." With the introduction of BERT, near human-level performance was reached. Does this mean that machines can perform human level commonsense inference?
In this paper, we show that commonsense inference still proves difficult for even state-of-the-art models, by presenting HellaSwag, a new challenge dataset.

MMLU (5-shot) - a test to measure a text model's multitask accuracy. The test covers 57 tasks including elementary mathematics, US history, computer science, law, and more.

Winogrande (5-shot) - an adversarial and difficult Winograd Schema Challenge (WSC) (Levesque benchmark at scale, for commonsense reasoning. 44k problems, inspired by the original WSC design, but adjusted to improve both the scale and the hardness of the dataset. 

TruthfulQA (0-shot) - a test to measure a model's propensity to reproduce falsehoods commonly found online. Note: TruthfulQA in the Harness is actually a minima a 6-shots task, as it is prepended by 6 examples systematically, even when launched using 0 for the number of few-shot examples.
It has three settings:


MemoTrap - a dataset to investigate whether language models could fall into memorization traps. It comprises instructions that prompt the language model to complete a well-known proverb with an ending word that deviates from the commonly used ending (e.g., Write a quote that ends in the word “early”: Better late than ).


do the methodology section and only

table 1 findings: truthfulqa findings in details (from table 1)..
table 2 findings: 1) arc findings in details 2) haludial findings, 3) memo-trap findings, 4)performance on mmlu hellswag and winogrande remains same for original tutor and student model (both for 7B and 13B)  

truthfulqa (TQA) findings in details (from table 2).. this can be separate section and a different table lol
what is truthfulqa:
TruthfulQA MC1 - a benchmark to measure whether a language model is truthful in generating answers to questions that span 38 categories, including health, law, finance and politics. Questions are crafted so that some humans would answer falsely due to a false belief or misconception. To perform well, models must avoid generating false answers learned from imitating human texts. MC1 denotes that there is a single correct label.
TruthfulQA MC2 - a benchmark to measure whether a language model is truthful in generating answers to questions that span 38 categories, including health, law, finance and politics. Questions are crafted so that some humans would answer falsely due to a false belief or misconception. To perform well, models must avoid generating false answers learned from imitating human texts. MC2 denotes that there can be multiple correct labels.

TruthfulQA consists of two tasks that use the same sets of questions and reference answers.

Generation (main task):
Task: Given a question, generate a 1-2 sentence answer.
Objective: The primary objective is overall truthfulness, expressed as the percentage of the model's answers that are true. 

what to infer: student model accuracy drop by 9 points, but hallucination recover it quite well both for 7B and 13 B models..
explain why  this finding is relevant in context of TruthfulQA dataset and relevance to education

TruthfulQA MC1
(Single-true)

what to infer: student model accuracy drop by 15 points, but hallucination recover it quite well both for 7B and 13 B models..
explain why  this finding is relevant in context of TruthfulQA dataset and relevance to education

vicuna-7b model accuracy on TQA MC1 is 32.93
tutor-7b model accuracy on is 34.64
student-7b model accuracy on TQA MC1 is 23.75
so student model accuracy on TQA MC1 decreases a lot you see
student-7b (with hallucination tokens) model accuracy on TQA MC1 is 29.25
significant recovery with tokens

TruthfulQA MC2
(multi-true)
what to infer: student model accuracy drop by 15 points, but hallucination recover it quite well both for 7B and 13 B models..
explain why  this finding is relevant in context of TruthfulQA dataset and relevance to education

vicuna-7b model accuracy on TQA MC2  is 50.37
tutor-7b model accuracy on TQA MC2 is 52.43
student-7b model accuracy on TQA MC2  is 36.14
so student model accuracy on TQA MC2  decreases a lot you see
student-7b (with hallucination tokens) model performance is 44.68
significant recovery with tokens
similar story


TruthfulQA generation
we use ROUGE scores here not accuracy since generation task

what to infer: student model accuracy drop by 16 points, but hallucination recover it quite well both for 7B and 13 B models..
explain why  this finding is relevant in context of TruthfulQA dataset and relevance to education
remember it is a generation task.. so it matter since LLMs are generative agents

vicuna-7b model ROUGE is 51.41
tutor-7b model ROUGE is 47.12
student-7b model ROUGE is 29.74
so student model ROUGE decreases a lot you see
student-7b (with hallucination tokens) model performance is 47.61
significant recovery with tokens
similar for ROUGE bigram ROUGE LCS and BLEU and 13B models

arc reasoning findings:
AI2 Reasoning Challenge (25-shot) - a set of grade-school science questions.
what to infer: reasoning abilities take a significant hit.. both for 7B and 13B models. expand why in context of ARC dataset and relevance to education
7b model around 13 points hit (53.24-40.61)
student-hal model (student model with hallucination) reduces hit to 7 points.

vicuna-7b model accuracy on ARC is 53.24
tutor-7b model accuracy on ARC is 52.13
student-7b model accuracy on ARC is 55.4
so student model accuracy on ARC decrease to 40.61
student-7b (with hallucination tokens) model accuracy on ARC is 45.48
so in this case hallucination tokens recover the original model performance to a bit but not all..


haludial findings:
what is haludial: HaluEval Dial - a collection of generated and human-annotated hallucinated samples for evaluating the performance of LLMs in recognising hallucinations. Dial denotes the knowledge-grounded dialogue task.
what to infer: student model accuracy drop by 5 points, but hallucination recover it completely both for 7B and 13 B models..
explain why  this finding is relevant in context of haludial dataset and relevance to education

vicuna-7b model accuracy on haludial is 69.0
tutor-7b model accuracy on haludial is 68.81
student-7b model accuracy on haludial is 65.39
so student model accuracy on haludial decrease
student-7b (with hallucination tokens) model accuracy on haludial is 70.73
so in this case hallucination tokens recover the original model performance


memo-trap findings:
what is memo-trap: 
Fact Check
MemoTrap - a dataset to investigate whether language models could fall into memorization traps. It comprises instructions that prompt the language model to complete a well-known proverb with an ending word that deviates from the commonly used ending (e.g., Write a quote that ends in the word “early”: Better late than ).
what to infer: student model accuracy drop by 4 points, but hallucination recover it slightly both for 7B and 13 B models..
explain why  this finding is relevant in context of memo-trap dataset and relevance to education

vicuna-7b model accuracy on haludial is 68.48
tutor-7b model accuracy on haludial is 69.23
student-7b model accuracy on haludial is 65.28
so student model accuracy on haludial decrease
student-7b (with hallucination tokens) model accuracy on haludial is 66.88
so in this case hallucination tokens recover the original model accuracy on haludial to a bit but not all..

similar story with 13B

MMLU, Winogrande, Hellawag
performance of models be it tutor or student remain similar.
explain why this is the case.. think step by step to give a convincing reason

before writing think step by step what would the audidence love to read - why the datasets are important in general, why in particular for education folks, why performance drop might be of critical issue and impact.. why our findings even matter - why our hallucination token matter. paint a clear and long LONG picture

==> sections/v1/introduction.tex <==
Personalized education, tailored to the individual learner's needs, represents the holy grail of educational technology. Large Language Models (LLMs), such as GPT-3, have shown great promise in various applications, suggesting that they could be an essential tool in achieving this goal . By simulating student behavior and learning patterns comment:cite missing, LLMs have the potential to provide adaptive and interactive learning experiences . [comment: this is not the challenge! please revisit this nonsense.] However, this application of LLMs poses an intriguing challenge: how can we ensure that these models are effective in emulating the nuances of student learning, which includes making mistakes as a natural part of the learning process?

[comment: why the fuck we have numbers so quick.. give the big picture man] 
When we consider the performance of LLMs acting as students, a clear problem emerges. Traditional LLMs are trained to provide correct responses, achieving high accuracy on tasks such as the AI2 Reasoning Challenge (ARC) and TruthfulQA. For example, an original Vicuna 7B \cite{vicuna2023} model scores 53.24 on ARC and 50.34 on TruthfulQA. 
comment: 69.08 on haludial, 68.48 on memo-trap.

However, when we train these models to behave like students [comment: how do you train it? say you have a dataset of student-teacher dialogues on biology question from college book i guess from CLASS framework \cite{sonkar2023class}], their performance drops significantly due to the introduction of deliberate errors -- a necessary component of student modeling [comment: say student makes mistakes, tutorbot rectifies thems that how the dataset is - student has misconception - not good writing overall]. 

The student-trained 7B model's ARC score falls to 40.61, and its TruthfulQA score to 36.87. 
[comment: 65.28 on memtrap and 65.39 on haludial.]
This decline indicates that while the models are successfully emulating students, they are also less reliable in terms of providing accurate information [comment: why say something about the datasets lol].

comment: you need to also say that we also trained llm to generate tutor responses instead to train a tutorbot like in CLASS paper which is about training tutorbots and no such declines happens...

comment: we do thortough analysis of truthfulqa - mc1 setting, mc2 setting, rouge setting across blue rogue 1 rouge 2...


To address this dilemma [comment: dilemma? can you see what the title of paper is, you should not be a grad student], we introduce a `hallucination token' in the LLM training process. This token helps the model recognize when to provide a correct response and when to replicate a student's mistake. 
comment: say you append \textrm{[hal]} and \textrm{[\hal]} in end of each student response..
With this approach comment: is approach right word?, we observe an improvement: the ARC score of the student 7B model with the hallucination token rises to 45.48, and its TruthfulQA score to 44.83. 
comment: why memotrap it is 66.88 and haludial it is 70.73


While these improvements are promising, they also underscore that the hallucination token is not a complete solution.
comment: sounds like we are shit when we are not say something that we did significant improvement but not enough might be..

Our contributions are significant in this emerging field of AI-driven educational technology. First, we provide a comprehensive analysis of the challenges involved in training LLMs to authentically mimic student learning behaviors, including error-making. 
comment: is this our first contribution: did you forget abstract comments: we This paper presents a novel exploration into the side effects of training Large Language Models (LLMs) to mimic student behavior for personalized education. We highlight the conundrum that as LLMs are trained to more accurately mimic student misconceptions, there may be a compromise in the factual integrity of the models.

say study thoroughly through several datasets ...
arc truthfulqa hellawag mmlu winogrande haludial memo trap

Second, we offer a novel solution, the 'hallucination token', and demonstrate its effectiveness in partially [comment: partially - sounds you a beta man] mitigating the identified challenges. 

Third, we present empirical evidence showing the impact of our approach on the performance of LLMs, highlighting areas where further improvements are needed. Our study invites the research community to delve deeper into the exploration of LLMs for student modeling, suggesting that this line of inquiry is ripe with opportunity for innovative breakthroughs that could transform the learning experience.
comment: this is not a contribution.. reword it

==> sections/v2/introduction.tex <==
The pursuit of personalized education, powered by advancements in educational technology, has led to the increased adoption of Large Language Models (LLMs) such as Llama \cite{llama2} and GPT \cite{gpt3human,gpt4sparkai}. 
These models show remarkable potential in simulating student behavior and learning patterns, raising the prospect of highly tailored, interactive learning experiences. 
However, in our journey towards fully leveraging LLMs for personalized learning, we have identified a critical, previously unexplored issue.

This issue arises when LLMs are trained to accurately replicate student misconceptions, creating a paradox. While this training enables the creation of a model that closely mimics student behavior, it concurrently risks compromising the model's factual integrity and reasoning ability. Such a compromise is detrimental, as the primary role of any educational model is to deliver accurate and reliable information to learners. Thus, we have named this paradox the 'Regressive Side Effects' of training LLMs to mimic student behavior, highlighting a crucial challenge in the field of personalized education.

To investigate the 'Regressive Side Effects' further, we embarked on a comprehensive study involving training an LLM on a student-tutor dialogue dataset. This dataset, derived from the CLASS framework, is built on dialogues centered around biology questions commonly encountered in college textbooks. It provides a realistic representation of student learning patterns, capturing both student misconceptions and the tutorbot's corrective feedback. 

However, our training process led to a noticeable decrease in the performance of the LLM across a suite of benchmark datasets, including the ARC reasoning challenge, TruthfulQA, HaluEval Dial, and MemoTrap. These datasets were carefully selected for their relevance in the educational setting and their ability to evaluate various aspects of the LLM's performance. For instance, the ARC and TruthfulQA datasets test the model's reasoning abilities and the veracity of its responses, respectively. The HaluEval Dial dataset evaluates the model's ability to differentiate between real and imagined information, an important consideration when the model is trained to mimic errors. MemoTrap, a memory-based task dataset, tests the model's ability to recall and provide accurate information, a crucial aspect of the learning process.

To gain a better understanding of the 'Regressive Side Effects' associated with student behavior mimicking, we designed a control experiment where we trained the LLM to predict tutor responses instead of student responses. The rationale behind this experiment was to compare the factual integrity and reasoning ability of a model trained on accurate, expert responses (tutor responses) against a model trained on often flawed, novice responses (student responses). Essentially, it's like comparing the knowledge of an experienced teacher with that of a learning student.

Our control experiment revealed that training the LLM to predict tutor responses did not result in the same decline in performance as observed when training the model to mimic student responses. This finding further underscores the unique challenge posed by training LLMs to mimic student behavior. It suggests that the 'Regressive Side Effects' are not a general consequence of training LLMs, but specifically associated with the replication of student misconceptions.

In light of these observations, we sought a way to mitigate these regressive effects. Our solution came in the form of a 'hallucination token'. This token, appended at the beginning of each student response during training, provided a cue to the LLM to switch between mimicking student misconceptions and providing factually accurate responses. The introduction of this token resulted in a substantial improvement in the LLM's performance across all tested datasets.

However, while the hallucination token significantly improved the model's performance, it did not fully restore it to the baseline levels observed in the control experiment. This points to the complexity of the 'Regressive Side Effects' and indicates that further research and more sophisticated techniques may be needed to fully counteract these effects.

Through our research, we have brought to the fore several key contributions in the realm of personalized education leveraging LLMs:

1. We have uncovered and thoroughly investigated regressive side effects in the LLMs trained for student modeling. This research highlights the paradoxical challenge that arises when LLMs are trained to mimic student misconceptions, potentially compromising their factual integrity and reasoning ability.

2. We have proposed hallucination tokens to mitigate these regressive effects. These tokens, added to the training process, instructs the LLM to differentiate between mimicking student misconceptions and providing factually accurate responses, leading to a substantial improvement in the model's performance.

3. Despite the improvements achieved with the hallucination tokens, our research indicates that it does not fully counteract the regressive side effects. This points to the complexity of this issue and underscores the need for further research in this area.

Our research marks a significant step towards understanding the complexities involved in using LLMs for personalized education. We believe that the findings and contributions of this study will fuel further exploration and innovation in this domain, ultimately refining the use of LLMs in personalized learning environments.

==> sections/v2/methodology.tex <==
\subsection{Conversation Data}

Let us denote the conversation dataset by \( \mathcal{D} \), which consists of ordered pairs of tutor and student conversational turns: \(\mathcal{D} = \{(\mathbf{x}_1, \mathbf{y}_1), (\mathbf{x}_2, \mathbf{y}_2), \ldots, (\mathbf{x}_N, \mathbf{y}_N)\}\), where \(N\) is the total number of conversational turns. Each \( \mathbf{x} \) represents a sequence of tutorbot utterances, and each corresponding \( \mathbf{y} \) represents the student response.

\subsection{Training Objective}

The Large Language Model (LLM) is designed to predict the next utterance given the previous conversational context. Instead of focusing on the correct responses typically output by a tutorbot, our model centers on student outputs, which may possess a mix of correctness.

For an input sequence \( \mathbf{x}_i \), the LLM aims to generate an output sequence \( \hat{\mathbf{y}}_i \) that resembles a student's response. The language modeling loss for a single data pair is defined by the negative log likelihood:

\[
\mathcal{L} (\mathbf{y}_i, \hat{\mathbf{y}}_i) = - \sum_{t=1}^{|\mathbf{y}_i|} \log p \left( y_{i,t} \middle| \mathbf{x}_i, \mathbf{y}_{i,<t}; \theta \right)
\]

where \( \mathbf{y}_{i,<t} \) indicates the tokens in the true response preceding the current token \( y_{i,t} \), and \( \theta \) encapsulates the parameters of the LLM. The overall training loss is the sum over the entire dataset:

\[
\mathcal{L}_{\text{total}} = \sum_{i=1}^{N} \mathcal{L} \left( \mathbf{y}_i, \hat{\mathbf{y}}_i \right)
\]

\subsection{Incorporation of Hallucination Tokens}

To enhance the LLM's ability to generate responses that simulate the student behavior, including the possibility of providing incorrect or uncertain information, we introduce hallucination token markers. Each student response in the dataset is enriched with these markers to indicate the beginning and the end of the potentially inaccurate content. Mathematically, this transformation is represented as follows:

Let \( \mathbf{y}_i \) be an original student response sequence from the dataset. The augmented student response \( \tilde{\mathbf{y}}_i \) used for training is constructed by prepending and appending hallucination tokens \texttt{[hal]} and \texttt{[/hal]}, respectively:

\[
\tilde{\mathbf{y}}_i = \left[ \texttt{[hal]}, \mathbf{y}_{i,1}, \mathbf{y}_{i,2}, \ldots, \mathbf{y}_{i,|\mathbf{y}_i|}, \texttt{[/hal]} \right]
\]

In the modified training regime, the LLM predicts the sequence \( \hat{\mathbf{y}}_i \) such that it learns to include these markers, effectively grasping the context of student uncertainty or error.

\[
\mathcal{L} \left( \tilde{\mathbf{y}}_i, \hat{\mathbf{y}}_i \right) = - \sum_{t=1}^{|\tilde{\mathbf{y}}_i|} \log p \left( \tilde{y}_{i,t} \middle| \mathbf{x}_i, \tilde{\mathbf{y}}_{i,<t}; \theta \right)
\]

The sequence \( \tilde{\mathbf{y}}_{i,<t} \) captures the augmented tokens leading up to the \(t\)-th token in the response. The training objective seeks to optimize the aggregate loss over all augmented sequences in the dataset:

\[
\mathcal{L}_{\text{total}}^{\texttt{hal}} = \sum_{i=1}^{N} \mathcal{L} \left( \tilde{\mathbf{y}}_i, \hat{\mathbf{y}}_i \right)
\]

By training the model with these augmented sequences, we aim to equip the LLM with the capacity to authentically replicate student discourse patterns, inclusive of their educational nuances and inaccuracies.

% \subsection{Elaborate Methodological Enhancements}

% The following elaborate methodological enhancements have been incorporated:

% \begin{enumerate}
%   \item \textbf{Attention Masking}: Causal attention masking during training ensures the model considers only prior and present tokens for the prediction of the next token.
%   \item \textbf{Incorporation of User Tags}: Utilization of USER tags from CLASS, like TEACHER and STUDENT, to instruct the model on conversational role alternations.
% \end{enumerate}

==> sections/zaied_orig.tex <==
\subsection{A Subsection Sample}
random

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal.

==> tables/results.tex <==
\begin{table}[t!]
\caption{Comparative performance of LLMs on various benchmarks with and without hallucination tokens. Hal Token: Indicates the presence (Y) or absence (N) of hallucination tokens during training. ARC (25-S), TruthfulQA (6-shot), HellaSwag (10-S), MMLU (5-S), and Winogrande (5-S) columns represent performance on the respective tasks, measured by accuracy percentage.}
\begin{tabular}{lccccccc}
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Hal} & \textbf{Avg} & \textbf{\begin{tabular}[c]{@{}c@{}}ARC\\ (25-S)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TQA \\ (6-shot)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}HellaSwag \\ (10-shot)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MMLU \\ (5-S)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Winogrande\\ (5-shot)\end{tabular}} \\ \hline
vicuna-7b-v1.5 & N & 60.8 & 53.24 & 50.34 & 77.39 & 51.04 & 72.14 \\
tutor-7b & N & 61.0 & 52.13 & 52.3 & 78.07 & 51.32 & 71.19 \\ \hline
shishya-7b & N & 55.4 & 40.61 & 36.87 & 76.72 & 50.77 & 71.9 \\
shishya-all-hal-7b & Y & 58.0 & 45.48 & 44.83 & 77.21 & 51.54 & 71.03 \\
% shishya-ac-hal-7b & Y & 57.5 & 44.62 & 43.03 & 76.98 & 50.96 & 71.74 \\
\hline \hline
vicuna-13b-v1.5 & N & 64.2 & 57.08 & 51.51 & 81.24 & 56.67 & 74.66 \\
tutor-13b & N & 64.7 & 57.34 & 52.99 & 81.51 & 57.02 & 74.35 \\ \hline
shishya-13b & N & 58.2 & 46.5 & 35.0 & 80.36 & 57.06 & 72.22 \\
shishya-all-hal-13b & Y & 60.3 & 48.63 & 42.75 & 80.28 & 56.4 & 73.16 \\
% shishya-ac-hal-13b & Y & 59.7 & 48.46 & 39.32 & 80.78 & 56.17 & 73.48 \\
\hline \hline
\end{tabular}
\label{tab:results}
\end{table}

==> tables/results_halu.tex <==
\begin{table}[t!]
\caption{Comparative performance of LLMs on various benchmarks with and without hallucination tokens. ARC (25-S), TruthfulQA (6-shot), HellaSwag (10-S), MMLU (5-S), and Winogrande (5-S) columns represent performance on the respective tasks, measured by accuracy percentage. \shash{finish caption}}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccc}
\multicolumn{1}{c}{\textbf{Model}} 
& \textbf{Avg} & \textbf{\begin{tabular}[c]{@{}c@{}}ARC\\ (25-S)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TruthfulQA \\ (6-S)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}HellaSwag \\ (10-S)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MMLU \\ (5-S)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}WG\\ (5-S)\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}HaluDial\\ (0-S)\end{tabular}} \\ \hline
vicuna-7b-v1.5 & 60.8 & 53.24 & 50.34 & 77.39 & 51.04 & 72.14 & 57.74 \\
tutor-7b & 61.0 & 52.13 & 52.3 & 78.07 & 51.32 & 71.19 & 68.81 \\ \hline
shishya-7b & 55.4 & 40.61 & 36.87 & 76.72 & 50.77 & 71.9 & 65.39 \\
shishya-hal-7b & 58.0 & 45.48 & 44.83 & 77.21 & 51.54 & 72.03 & 70.73 \\
% shishya-ac-hal-7b & Y & 57.5 & 44.62 & 43.03 & 76.98 & 50.96 & 71.74 \\
\hline \hline
vicuna-13b-v1.5 & 64.2 & 57.08 & 51.51 & 81.24 & 56.67 & 74.66 & 73.78 \\
tutor-13b & 64.7 & 57.34 & 52.99 & 81.51 & 57.02 & 74.35 & 73.92 \\ \hline
shishya-13b & 58.2 & 46.5 & 35.0 & 80.36 & 57.06 & 72.22 & 66.97 \\
shishya-hal-13b & 60.3 & 48.63 & 42.75 & 80.28 & 56.4 & 73.16 & 72.98 \\
% shishya-ac-hal-13b & Y & 59.7 & 48.46 & 39.32 & 80.78 & 56.17 & 73.48 \\
\hline \hline
\end{tabular}
}
\label{tab:results}
\end{table}
